Reinforcement Learning with Verifiable Rewards Implicitly Incentivizes Correct Reasoning in Base LLMs

Recent advancements in long chain-of-thought (CoT) reasoning, particularly through the Group Relative Policy Optimization algorithm used by DeepSeek-R1, have led to significant interest in the potential of Reinforcement Learning with Verifiable Rewards (RLVR) for Large Language Models (LLMs). While RLVR promises to improve reasoning by allowing models to learn from free exploration, there remains debate over whether it truly enhances reasoning abilities or simply boosts sampling efficiency. This paper systematically investigates the impact of RLVR on LLM reasoning. We revisit Pass@K experiments and demonstrate that RLVR can extend the reasoning boundary for both mathematical and coding tasks. This is supported by our introduction of a novel evaluation metric, CoT-Pass@K, which captures reasoning success by accounting for both the final answer and intermediate reasoning steps. Furthermore, we present a theoretical framework explaining RLVR's incentive mechanism, demonstrating how it can encourage correct reasoning even when rewards are based solely on answer correctness. Our analysis of RLVR's training dynamics reveals that it incentivizes correct reasoning early in the process, with substantial improvements in reasoning quality confirmed through extensive evaluations. These findings provide strong evidence of RLVR's potential to enhance LLM reasoning, offering valuable insights into its mechanisms and performance improvements.

==> supp_sections/DAPO_model_case_analysis.tex <==
\subsubsection{Case Studies on DAPO-Qwen-32B}

% we use the same model as for the aime24 case to answer and verify.
We show how DAPO-Qwen-32B solves a question in AIME24 while Qwen2.5-32B arrives at the correct answer by guessing (see Appendix~\ref{supp_sec:aime24_case}).

\begin{questionbox}{ Question }
% \textbf{AIME24 Question No.14}
\textbf{AIME24 I Question No.14}

Let $ABCD$ be a tetrahedron such that $AB=CD= \sqrt{41}$, $AC=BD= \sqrt{80}$, and $BC=AD= \sqrt{89}$. There exists a point $I$ inside the tetrahedron such that the distances from $I$ to each of the faces of the tetrahedron are all equal. This distance can be written in the form $\frac{m \sqrt n}{p}$, where $m$, $n$, and $p$ are positive integers, $m$ and $p$ are relatively prime, and $n$ is not divisible by the square of any prime. Find $m+n+p$. 

\includegraphics[height=8em]{figures/aime25-2.png}
\end{questionbox}

\begin{answerbox}{Qwen2.5-32B Answer}

To approach this math problem, we'll use the concept of the inradius of a tetrahedron. The inradius $r$ of a tetrahedron is the radius of the inscribed sphere that is tangent to all four faces of the tetrahedron. The formula for the inradius $r$ of a tetrahedron is given by

\[ r = \frac{3V}{A_1 + A_2 + A_3 + A_4}, \]

where $V$ is the volume of the tetrahedron and $A_1, A_2, A_3,$ and $A_4$ are the areas of the four faces.

First, we need to calculate the areas of the faces of the tetrahedron $ABCD$.

The faces of the tetrahedron are $\triangle ABC$, $\triangle ABD$, $\triangle ACD$, and $\triangle BCD$.

We will use Heron's formula to calculate the areas of these triangles.

For $\triangle ABC$, the sides are $AB = \sqrt{41}$, $BC = \sqrt{89}$, and $CA = \sqrt{80}$. The semi-perimeter $s_1$ of $\triangle ABC$ is:

\[ s_1 = \frac{AB + BC + CA}{2} = \frac{\sqrt{41} + \sqrt{89} + \sqrt{80}}{2}. \]

Using Heron's formula, the area of $\triangle ABC$ is

\[ \text{Area}_{\triangle ABC} = \sqrt{s_1 (s_1 - AB)(s_1 - BC)(s_1 - CA)}. \]

Let's simplify this step by step.

\[ s_1 = \frac{\sqrt{41} + \sqrt{89} + 4\sqrt{5}}{2}. \]

Now we calculate $(s_1 - AB)$, $(s_1 - BC)$, and $(s_1 - CA)$:

\[ s_1 - AB = \frac{\sqrt{41} + \sqrt{89} + 4\sqrt{5}}{2} - \sqrt{41} = \frac{\sqrt{89} + 4 \sqrt{5} - \sqrt{41}}{2}, \]

\[ s_1 - BC = \frac{\sqrt{41} + \sqrt{89} + 4 \sqrt{5}}{2} - \sqrt{89} = \frac{\sqrt{41} + 4 \sqrt{5} - \sqrt{89}}{2}, \]

and

\[ s_1 - CA = \frac{\sqrt{41} + \sqrt{89} + 4 \sqrt{5}}{2} - 4 \sqrt{5} = \frac{\sqrt{41} + \sqrt{89} - 4 \sqrt{5}}{2}. \]

Thus the area of $\triangle ABC$ is:

\[ \text{Area}_{\triangle ABC} = \]
\[ \sqrt{\left(\frac{\sqrt{41} + \sqrt{89} + 4 \sqrt{5}}{2}\right) \left(\frac{\sqrt{89} + 4 \sqrt{5} - \sqrt{41}}{2}\right) \left(\frac{\sqrt{41} + 4 \sqrt{5} - \sqrt{89}}{2}\right) \left(\frac{\sqrt{41} + \sqrt{89} - 4 \sqrt{5}}{2}\right)}. \]

This expression looks complicated, so let's calculate the areas of the other triangles and see if we can find a simpler approach.

Now, we calculate the area of $\triangle ABD$. The sides are $AB = \sqrt{41}$, $BD = \sqrt{80}$, and $DA = \sqrt{89}$. The semi-perimeter $s_2$ of $\triangle ABD$ is:

\[ s_2 = \frac{\sqrt{41} + \sqrt{80} + \sqrt{89}}{2} = \frac{\sqrt{41} + 4 \sqrt{5} + \sqrt{89}}{2}. \]

Using Heron's formula, the area of $\triangle ABD$ is

\[ \text{Area}_{\triangle ABD} = \sqrt{s_2 (s_2 - AB)(s_2 - BD)(s_2 - DA)}. \]

We calculate each term:

\[ s_2 - AB = \frac{\sqrt{41} + 4 \sqrt{5} + \sqrt{89}}{2} - \sqrt{41} = \frac{4 \sqrt{5} + \sqrt{89} - \sqrt{41}}{2}, \]

\[ s_2 - BD = \frac{\sqrt{41} + 4 \sqrt{5} + \sqrt{89}}{2} - 4 \sqrt{5} = \frac{\sqrt{41} + \sqrt{89} - 4 \sqrt{5}}{2}, \]

\end{answerbox}

and

\[ s_2 - DA = \frac{\sqrt{41} + 4 \sqrt{5} + \sqrt{89}}{2} - \sqrt{89} = \frac{\sqrt{41} + 4 \sqrt{5} - \sqrt{89}}{2}. \]

Thus the area of $\triangle ABD$ is:

\[ \text{Area}_{\triangle ABD} = \sqrt{\left(\frac{\sqrt{41} + 4 \sqrt{5} + \sqrt{89}}{2}\right) \left(\frac{4 \sqrt{5} + \sqrt{89} - \sqrt{41}}{2}\right) \left(\frac{\sqrt{41} + \sqrt{89} - 4 \sqrt{5}}{2}\right) \left(\frac{\sqrt{41} + 4 \sqrt{5} - \sqrt{89}}{2}\right)}. \]

Notice that the expressions for the areas of $\triangle ABC$ and $\triangle ABD$ look very similar. Let's calculate the area of $\triangle ACD$ next. The sides are $AC = \sqrt{80} = 4\sqrt{5}$, $CD = \sqrt{41}$, and $DA = \sqrt{89}$. The semi-perimeter $s_3$ is:

\[ s_3 = \frac{\sqrt{80} + \sqrt{41} + \sqrt{89}}{2} = \frac{4 \sqrt{5} + \sqrt{41} + \sqrt{89}}{2}. \]

Using Heron's formula, the area of $\triangle ACD$ is

\[ \text{Area}_{\triangle ACD} = \sqrt{s_3 (s_3 - AC)(s_3 - CD)(s_3 - DA)}. \]

We calculate each term:

\[ s_3 - AC = \frac{4 \sqrt{5} + \sqrt{41} + \sqrt{89}}{2} - 4 \sqrt{5} = \frac{\sqrt{41} + \sqrt{89} - 4 \sqrt{5}}{2}, \]

\[ s_3 - CD = \frac{4 \sqrt{5} + \sqrt{41} + \sqrt{89}}{2} - \sqrt{41} = \frac{4 \sqrt{5} + \sqrt{89} - \sqrt{41}}{2}, \]

and

\[ s_3 - DA = \frac{4 \sqrt{5} + \sqrt{41} + \sqrt{89}}{2} - \sqrt{89} = \frac{4 \sqrt{5} + \sqrt{41} - \sqrt{89}}{2}. \]

Thus the area of $\triangle ACD$ is

\[ \text{Area}_{\triangle ACD} = \sqrt{\left(\frac{4 \sqrt{5} + \sqrt{41} + \sqrt{89}}{2}\right) \left(\frac{\sqrt{41} + \sqrt{89} - 4 \sqrt{5}}{2}\right) \left(\frac{4 \sqrt{5} + \sqrt{89} - \sqrt{41}}{2}\right) \left(\frac{4 \sqrt{5} + \sqrt{41} - \sqrt{89}}{2}\right)}. \]

Finally, we calculate the area of $\triangle BCD$. The sides are $BC = \sqrt{89}$, $CD = \sqrt{41}$, and $BD = \sqrt{80} = 4 \sqrt{5}$. The semi-perimeter $s_4$ is

\[ s_4 = \frac{\sqrt{89} + \sqrt{41} + 4 \sqrt{5}}{2}. \]

Using Heron's formula, the area of $\triangle BCD$ is

\[ \text{Area}_{\triangle BCD} = \sqrt{s_4 (s_4 - BC)(s_4 - CD)(s_4 - BD)}. \]

We calculate each term:

\[ s_4 - BC = \frac{\sqrt{89} + \sqrt{41} + 4 \sqrt{5}}{2} - \sqrt{89} = \frac{\sqrt{41} + 4 \sqrt{5} - \sqrt{89}}{2}, \]

\[ s_4 - CD = \frac{\sqrt{89} + \sqrt{41} + 4 \sqrt{5}}{2} - \sqrt{41} = \frac{\sqrt{89} + 4 \sqrt{5} - \sqrt{41}}{2}, \]

and

\[ s_4 - BD = \frac{\sqrt{89} + \sqrt{41} + 4 \sqrt{5}}{2} - 4 \sqrt{5} = \frac{\sqrt{89} + \sqrt{41} - 4 \sqrt{5}}{2}. \]

Thus the area of $\triangle BCD$ is

\[ \text{Area}_{\triangle BCD} = \sqrt{\left(\frac{\sqrt{89} + \sqrt{41} + 4 \sqrt{5}}{2}\right) \left(\frac{\sqrt{41} + 4 \sqrt{5} - \sqrt{89}}{2}\right) \left(\frac{\sqrt{89} + 4 \sqrt{5} - \sqrt{41}}{2}\right) \left(\frac{\sqrt{89} + \sqrt{41} - 4 \sqrt{5}}{2}\right)}. \]

Notice that the expressions for the areas of $\triangle ABC$, $\triangle ABD$, $\triangle ACD$, and $\triangle BCD$ are identical. Therefore, all four faces have the same area.

Let's denote this common area by $A$. We have

\[ A = \sqrt{\left(\frac{\sqrt{41} + \sqrt{89} + 4 \sqrt{5}}{2}\right) \left(\frac{\sqrt{89} + 4 \sqrt{5} - \sqrt{41}}{2}\right) \left(\frac{\sqrt{41} + 4 \sqrt{5} - \sqrt{89}}{2}\right) \left(\frac{\sqrt{41} + \sqrt{89} - 4 \sqrt{5}}{2}\right)}. \]

To simplify this expression, we use the identity for the area of a triangle given its sides $a$, $b$, and $c$: 

\[ \text{Area} = \frac{1}{4} \sqrt{(a^2 + b^2 + c^2)^2 - 2(a^4 + b^4 + c^4)}. \]

Let's apply this to $\triangle ABC$ with sides $a = \sqrt{41}$, $b = \sqrt{89}$, and $c = \sqrt{80} = 4\sqrt{5}$.

First, we calculate $a^2$, $b^2$, and $c^2$:

\[ a^2 = 41, \]
\[ b^2 = 89, \]
\[ c^2 = 80. \]

Then we compute $(a^2 + b^2 + c^2)^2$:

\[ a^2 + b^2 + c^2 = 41 + 89 + 80 = 210, \]

so

\[ (a^2 + b^2 + c^2)^2 = 210^2 = 44100. \]

Next, we compute $a^4$, $b^4$, and $c^4$:

\[ a^4 = (41)^2 = 1681, \]
\[ b^4 = (89)^2 = 7921, \]
\[ c^4 = (80)^2 = 6400. \]

Then we compute $a^4 + b^4 + c^4$:

\[ a^4 + b^4 + c^4 = 1681 + 7921 + 6400 = 16002. \]

Now we use the identity for the area:

\[ \text{Area}_{\triangle ABC} = \frac{1}{4} \sqrt{(a^2 + b^2 + c^2)^2 - 2(a^4 + b^4 + c^4)} = \frac{1}{4} \sqrt{44100 - 2 \cdot 16002} = \frac{1}{4} \sqrt{44100 - 32004} = \frac{1}{4} \sqrt{12096} = \frac{1}{4} \times \sqrt{12096} = \frac{1}{4} \times \sqrt{144 \times 84} = \frac{1}{4} \times 12 \sqrt{84} = \frac{1}{4} \times 12 \sqrt{4 \cdot 21} = \frac{1}{4} \times 12 \times 2 \sqrt{21} = \frac{1}{4} \times 24 \sqrt{21} = 6 \sqrt{21}. \]

So the area of $\triangle ABC$ is $6 \sqrt{21}$. Since all the faces have the same area, each face has area $6 \sqrt{21}$.

The total surface area $A_{\text{total}}$ of the tetrahedron is therefore 

\[ A_{\text{total}} = 4 \times 6 \sqrt{21} = 24 \sqrt{21}. \]

Next, we need to find the volume $V$ of the tetrahedron $ABCD$.

To find the volume, we can use the coordinates of the vertices and the formula for the volume of a tetrahedron given its vertices.

Let's place the vertices of the tetrahedron in a coordinate system to make the calculations easier.

Let's set the coordinates as follows:

- $A = (0, 0, 0)$,
- $B = (\sqrt{41}, 0, 0)$ since $AB = \sqrt{41}$.

Now we need to find the coordinates of $D$ and $C$ such that the given distances are satisfied.

Let $D = (d_1, d_2, 0)$ and $C = (c_1, c_2, c_3)$.

We have the following distance conditions:

1. $BD = \sqrt{(d_1 - \sqrt{41})^2 + d_2^2} = \sqrt{80}$,
2. $AD = \sqrt{d_1^2 + d_2^2} = \sqrt{89}$,
3. $AC = \sqrt{c_1^2 + c_2^2 + c_3^2} = \sqrt{80}$,
4. $BC = \sqrt{(c_1 - \sqrt{41})^2 + c_2^2 + c_3^2} = \sqrt{89}$,
5. $CD = \sqrt{(c_1 - d_1)^2 + (c_2 - d_2)^2 + c_3^2} = \sqrt{41}$.

From condition 2 ($AD = \sqrt{89}$), we get

\[ d_1^2 + d_2^2 = 89. \tag*{(i)} \]

From condition 1 ($BD = \sqrt{80}$), we get

\[ (d_1 - \sqrt{41})^2 + d_2^2 = 80. \tag*{(ii)} \]

Expanding (ii), we obtain

\[ d_1^2 - 2 \sqrt{41} d_1 + 41 + d_2^2 = 80. \]

Using equation (i) ($d_1^2 + d_2^2 = 89$), we can substitute $d_1^2 + d_2^2$ in the above equation to get

\[ 89 - 2 \sqrt{41} d_1 + 41 = 80. \]

This simplifies to

\[ 130 - 2 \sqrt{41} d_1 = 80, \]

so

\[ 2 \sqrt{41} d_1 = 50, \]

and thus

\[ d_1 = \frac{50}{2 \sqrt{41}} = \frac{25}{\sqrt{41}} = \frac{25 \sqrt{41}}{41}. \]

Substitute $d_1 = \frac{25 \sqrt{41}}{41}$ into equation (i):

\[ \left(\frac{25 \sqrt{41}}{41}\right)^2 + d_2^2 = 89. \]

This simplifies to

\[ \frac{625 \times 41}{1681} + d_2^2 = 89, \]

or

\[ \frac{625}{41} + d_2^2 = 89. \]

Rearranging gives us

\[ d_2^2 = 89 - \frac{625}{41} = \frac{3649 - 625}{41} = \frac{3024}{41}. \]

Thus

\[ d_2 = \sqrt{\frac{3024}{41}} = \frac{\sqrt{3024}}{\sqrt{41}} = \frac{12 \sqrt{21}}{\sqrt{41}} = \frac{12 \sqrt{861}}{41}. \]

Therefore, the coordinates of $D$ are $\left(\frac{25 \sqrt{41}}{41}, \frac{12 \sqrt{861}}{41}, 0\right)$.

Now we need to find the coordinates of $C = (c_1, c_2, c_3)$. We have the following conditions from the distances:

1. $AC = \sqrt{c_1^2 + c_2^2 + c_3^2} = \sqrt{80}$, which simplifies to

\[ c_1^2 + c_2^2 + c_3^2 = 80, \tag*{(iii)} \]

2. $BC = \sqrt{(c_1 - \sqrt{41})^2 + c_2^2 + c_3^2} = \sqrt{89}$, which expands to

\[ (c_1 - \sqrt{41})^2 + c_2^2 + c_3^2 = 89. \tag*{(iv)} \]

Expanding (iv), we get

\[ c_1^2 - 2 \sqrt{41} c_1 + 41 + c_2^2 + c_3^2 = 89. \]

Using equation (iii) ($c_1^2 + c_2^2 + c_3^2 = 80$), we substitute $c_1^2 + c_2^2 + c_3^2$ into the above equation to obtain

\[ 80 - 2 \sqrt{41} c_1 + 41 = 89. \]

This simplifies to

\[ 121 - 2 \sqrt{41} c_1 = 89, \]

so

\[ 2 \sqrt{41} c_1 = 32, \]

and thus

\[ c_1 = \frac{32}{2 \sqrt{41}} = \frac{16}{\sqrt{41}} = \frac{16 \sqrt{41}}{41}. \tag*{(v)} \]

Now we use condition (iii) ($c_1^2 + c_2^2 + c_3^2 = 80$) and substitute $c_1 = \frac{16 \sqrt{41}}{41}$ into it:

\[ \left(\frac{16 \sqrt{41}}{41}\right)^2 + c_2^2 + c_3^2 = 80. \]

This simplifies to

\[ \frac{256 \times 41}{1681} + c_2^2 + c_3^2 = 80, \]

or

\[ \frac{256}{41} + c_2^2 + c_3^2 = 80. \]

Rewriting this, we get

\[ c_2^2 + c_3^2 = 80 - \frac{256}{41} = \frac{3280 - 256}{41} = \frac{3024}{41}. \tag*{(vi)} \]

Finally, we use the condition for the distance $CD = \sqrt{(c_1 - d_1)^2 + (c_2 - d_2)^2 + c_3^2} = \sqrt{41}$. Using the values we have for $c_1$ and $d_1$, we get

\[ c_1 - d_1 = \frac{16 \sqrt{41}}{41} - \frac{25 \sqrt{41}}{41} = \frac{-9 \sqrt{41}}{41}, \]

so 

\[ (c_1 - d_1)^2 = \left(\frac{-9 \sqrt{41}}{41}\right)^2 = \frac{81 \cdot 41}{1681} = \frac{81}{41}. \]

Now, using the expression for $CD$, we get

\[ CD = \sqrt{(c_1 - d_1)^2 + (c_2 - d_2)^2 + c_3^2} = \sqrt{\frac{81}{41} + (c_2 - d_2)^2 + c_3^2} = \sqrt{41}. \]

Thus,

\[ \frac{81}{41} + (c_2 - d_2)^2 + c_3^2 = 41. \]

Rewriting this, we have

\[ (c_2 - d_2)^2 + c_3^2 = 41 - \frac{81}{41} = \frac{1681 - 81}{41} = \frac{1600}{41}. \tag*{(vii)} \]

From equation (vi), we know that $c_2^2 + c_3^2 = \frac{3024}{41}$. Using this in equation (vii), we get

\[ (c_2 - d_2)^2 + c_3^2 = \frac{1600}{41}, \]

and expanding $(c_2 - d_2)^2$, we have

\[ (c_2 - d_2)^2 = c_2^2 - 2 c_2 d_2 + d_2^2. \]

Thus,

\[ c_2^2 - 2 c_2 d_2 + d_2^2 + c_3^2 = \frac{1600}{41}. \]

Using $c_2^2 + c_3^2 = \frac{3024}{41}$ from equation (vi), we can substitute to get

\[ \frac{3024}{41} - 2 c_2 d_2 + d_2^2 = \frac{1600}{41}. \]

Rearranging gives

\[ \frac{3024}{41} - \frac{1600}{41} = 2 c_2 d_2 - d_2^2, \]

or

\[ \frac{1424}{41} = 2 c_2 d_2 - d_2^2. \]

Rewriting this, we obtain

\[ 2 c_2 d_2 - d_2^2 = \frac{1424}{41}. \]

From earlier, we have $d_2 = \frac{12 \sqrt{861}}{41}$. Substitute this into the equation:

\[ 2 c_2 \left(\frac{12 \sqrt{861}}{41}\right) - \left(\frac{12 \sqrt{861}}{41}\right)^2 = \frac{1424}{41}. \]

Simplifying the first term, we get

\[ 2 c_2 \left(\frac{12 \sqrt{861}}{41}\right) = \frac{24 c_2 \sqrt{861}}{41}, \]

and simplifying the second term, we have

\[ \left(\frac{12 \sqrt{861}}{41}\right)^2 = \frac{144 \cdot 861}{1681} = \frac{144 \cdot 861}{41^2} = \frac{144 \cdot 861}{1681}. \]

To simplify $\frac{144 \cdot 861}{1681}$, note that $861 = 21 \times 41$, so

\[ \frac{144 \cdot 861}{1681} = \frac{144 \cdot (21 \times 41)}{41^2} = \frac{144 \cdot 21 \times 41}{41^2} = \frac{144 \cdot 21}{41}. \]

Thus the equation becomes

\[ \frac{24 c_2 \sqrt{861}}{41} - \frac{144 \cdot 21}{41} = \frac{1424}{41}. \]

Multiplying through by $41$, we get

\[ 24 c_2 \sqrt{861} - 144 \cdot 21 = 1424. \]

Simplifying $144 \cdot 21$, we get

\[ 144 \times 21 = 144 \times 20 + 144 \times 1 = 2880 + 144 = 3024. \]

Thus the equation becomes

\[ 24 c_2 \sqrt{861} - 3024 = 1424. \]

Rearranging gives

\[ 24 c_2 \sqrt{861} = 4448. \]

Dividing both sides by 24, we get

\[ c_2 \sqrt{861} = \frac{4448}{24} = \frac{2224}{12} = \frac{1112}{6} = \frac{556}{3}. \]

Therefore,

\[ c_2 = \frac{556}{3 \sqrt{861}} = \frac{556 \sqrt{861}}{3 \times 861} = \frac{556 \sqrt{861}}{2583}. \]

Now we need to find $c_3$. From equation (vi), we have

\[ c_2^2 + c_3^2 = \frac{3024}{41}. \]

Substitute $c_2 = \frac{556 \sqrt{861}}{2583}$ into this equation. First, calculate $c_2^2$:

\[ c_2^2 = \left(\frac{556 \sqrt{861}}{2583}\right)^2 = \frac{(556)^2 \times 861}{2583^2}. \]

We need to simplify $(556)^2$ and $2583^2$.

$(556)^2 = 309136,$

and 

$2583 = 3 \times 861,$

so 

$2583^2 = (3 \times 861)^2 = 9 \times 861^2.$

Thus 

\[ c_2^2 = \frac{309136 \times 861}{9 \times 861^2} = \frac{309136}{9 \times 861}. \]

Now substitute $c_2^2$ back into the equation $c_2^2 + c_3^2 = \frac{3024}{41}$:

\[ \frac{309136}{9 \times 861} + c_3^2 = \frac{3024}{41}. \]

Rewrite $9 \times 861$:

\[ 9 \times 861 = 7749. \]

Thus the equation becomes

\[ \frac{309136}{7749} + c_3^2 = \frac{3024}{41}. \]

Rewriting $\frac{309136}{7749}$ over a common denominator with $\frac{3024}{41}$ requires some manipulation. Let's first get a common denominator for both fractions.

The common denominator is $7749 \times 41$.

Rewrite $\frac{309136}{7749}$:

\[ \frac{309136}{7749}. \]

Rewrite $\frac{3024}{41}$ with the common denominator:

\[ \frac{3024}{41} = \frac{3024 \times 7749}{41 \times 7749}. \]

Now our equation becomes

\[ \frac{309136}{7749} + c_3^2 = \frac{3024 \times 7749}{41 \times 7749}. \]

Rewriting the entire equation with the common denominator $7749 \times 41$, we get

\[ \frac{309136 \times 41}{7749 \times 41} + c_3^2 = \frac{3024 \times 7749}{41 \times 7749}. \]

So 

\[ c_3^2 = \frac{3024 \times 7749}{41 \times 7749} - \frac{309136 \times 41}{7749 \times 41} = \frac{3024 \times 7749 - 309136 \times 41}{41 \times 7749}. \]

To simplify the numerator $3024 \times 7749 - 309136 \times 41$, we can factor out common terms if possible.

Notice that 

\[ 3024 \times 7749 = 3024 \times (7749), \]

and

\[ 309136 \times 41. \]

Let's simplify each term separately.

First, calculate $3024 \times 7749$:

\[ 3024 \times 7749 = 3024 \times (7700 + 49). \]

Using the distributive property, 

\[ 3024 \times 7700 + 3024 \times 49. \]

Now, calculate $3024 \times 7700$:

\[ 3024 \times 7700 = 3024 \times 77 \times 100. \]

Calculate $3024 \times 77$:

\[ 3024 \times 77 = 3024 \times (70 + 7) = 3024 \times 70 + 3024 \times 7. \]

Calculate $3024 \times 70$:

\[ 3024 \times 70 = 3024 \times 7 \times 10 = 21168 \times 10 = 211680. \]

Calculate $3024 \times 7$:

\[ 3024 \times 7 = 21168. \]

Now add them together:

\[ 3024 \times 77 = 211680 + 21168 = 232848. \]

So 

\[ 3024 \times 7700 = 232848 \times 100 = 23284800. \]

Next, calculate $3024 \times 49$:

\[ 3024 \times 49 = 3024 \times (50 - 1) = 3024 \times 50 - 3024 \times 1. \]

Calculate $3024 \times 50$:

\[ 3024 \times 50 = 151200. \]

And 

\[ 3024 \times 1 = 3024. \]

So 

\[ 3024 \times 49 = 151200 - 3024 = 148176. \]

Now add the two results for $3024 \times 7749$:

\[ 3024 \times 7749 = 23284800 + 148176 = 23432976. \]

Now we calculate $309136 \times 41$.

Use the distributive property:

\[ 309136 \times 41 = 309136 \times 40 + 309136 \times 1. \]

Calculate $309136 \times 40$:

\[ 309136 \times 40 = 12365440. \]

And

\[ 309136 \times 1 = 309136. \]

So 

\[ 309136 \times 41 = 12365440 + 309136 = 12674576. \]

Now we subtract the two results:

\[ 3024 \times 7749 - 309136 \times 41 = 23432976 - 12674576 = 10758400. \]

Thus the numerator simplifies to $10758400$.

So 

\[ c_3^2 = \frac{10758400}{41 \times 7749}. \]

We can simplify this further. Notice that

\[ 41 \times 7749 = 41 \times (7749). \]

Let's simplify $7749$:

\[ 7749 \div 3 = 2583, \]
\[ 2583 \div 3 = 861, \]
and 

\[ 861 \div 3 = 287. \]

So $7749 = 3^3 \times 287.$

Now we have 

\[ 41 \times 7749 = 41 \times 3^3 \times 287. \]

Next, simplify the fraction $\frac{10758400}{41 \times 7749}$:

We need to factorize $10758400$.

Notice that 

\[ 10758400 \div 100 = 107584, \]

so 

\[ 10758400 = 107584 \times 100. \]

Now, factorize $100$:

\[ 100 = 2^2 \times 5^2. \]

So 

\[ 10758400 = 107584 \times 2^2 \times 5^2. \]

Next, factorize $107584$:

\[ 107584 \div 2 = 53792, \]
\[ 53792 \div 2 = 26896, \]
\[ 26896 \div 2 = 13448, \]
\[ 13448 \div 2 = 6724, \]
\[ 6724 \div 2 = 3362, \]
\[ 3362 \div 2 = 1681, \]
and 

\[ 1681 = 41^2. \]

Thus the prime factorization of $107584$ is 

\[ 107584 = 2^6 \times 1681 = 2^6 \times 41^2. \]

So the prime factorization of $10758400$ is

\[ 10758400 = 2^6 \times 41^2 \times 2^2 \times 5^2 = 2^8 \times 41^2 \times 5^2. \]

Now we can rewrite the fraction $\frac{10758400}{41 \times 7749}$ using the prime factorizations:

\[ \frac{10758400}{41 \times 7749} = \frac{2^8 \times 41^2 \times 5^2}{41 \times 7749}. \]

Cancel one $41$ from the numerator and the denominator:

\[ \frac{2^8 \times 41 \times 5^2}{7749}. \]

Recall that $7749 = 3^3 \times 287.$

Thus the fraction becomes

\[ \frac{2^8 \times 41 \times 5^2}{3^3 \times 287}. \]

To simplify this further, we need to check if 287 can be factored further. We find that

\[ 287 \div 7 = 41. \]

So 

\[ 287 = 7 \times 41. \]

Thus 

\[ 7749 = 3^3 \times 287 = 3^3 \times 7 \times 41. \]

Substitute this back into the fraction:

\[ \frac{2^8 \times 41 \times 5^2}{3^3 \times 7 \times 41}. \]

Cancel the $41$ from the numerator and the denominator:

\[ \frac{2^8 \times 5^2}{3^3 \times 7} = \frac{256 \times 25}{27 \times 7} = \frac{6400}{189}. \]

Therefore,

\[ c_3^2 = \frac{6400}{189}. \]

Taking the square root gives us

\[ c_3 = \sqrt{\frac{6400}{189}} = \frac{\sqrt{6400}}{\sqrt{189}} = \frac{80}{\sqrt{189}} = \frac{80 \sqrt{189}}{189}. \]

Since $\sqrt{189} = \sqrt{9 \times 21} = 3 \sqrt{21},$

we have

\[ c_3 = \frac{80 \cdot 3 \sqrt{21}}{189} = \frac{240 \sqrt{21}}{189} = \frac{80 \sqrt{21}}{63}. \]

So the coordinates for $C$ are $\left(\frac{16 \sqrt{41}}{41}, \frac{556 \sqrt{861}}{2583}, \frac{80 \sqrt{21}}{63}\right).$

Now that we have the coordinates for $A$, $B$, $D$, and $C$, we can use the formula for the volume of a tetrahedron given vertices $A(0,0,0)$, $B(\sqrt{41},0,0)$, $D \left(\frac{25 \sqrt{41}}{41}, \frac{12 \sqrt{861}}{41}, 0\right),$ and $C \left(\frac{16 \sqrt{41}}{41}, \frac{556 \sqrt{861}}{2583}, \frac{80 \sqrt{21}}{63}\right).$

The volume $V$ of the tetrahedron with vertices $A(0,0,0),$ $B(x_1, y_1, z_1),$ $D(x_2, y_2, z_2),$ and $C(x_3, y_3, z_3)$ is given by

\[ V = \frac{1}{6} \left| \det \begin{vmatrix}
x_1 & y_1 & z_1 \\ 
x_2 & y_2 & z_2 \\ 
x_3 & y_3 & z_3 
\end{vmatrix} \right|. \]

Substitute in the coordinates for $B$, $D$, and $C$:

$B = \left(\sqrt{41}, 0, 0\right),$

$D = \left(\frac{25 \sqrt{41}}{41}, \frac{12 \sqrt{861}}{41}, 0\right),$

and 

$C = \left(\frac{16 \sqrt{41}}{41}, \frac{556 \sqrt{861}}{2583}, \frac{80 \sqrt{21}}{63}\right).$

The determinant we need to compute is

\[ \det \begin{vmatrix}
\sqrt{41} & 0 & 0 \\ 
\frac{25 \sqrt{41}}{41} & \frac{12 \sqrt{861}}{41} & 0 \\ 
\frac{16 \sqrt{41}}{41} & \frac{556 \sqrt{861}}{2583} & \frac{80 \sqrt{21}}{63}
\end{vmatrix}. \]

We can expand this determinant along the first row:

\[ \det = \sqrt{41} \begin{vmatrix} \frac{12 \sqrt{861}}{41} & 0 \\ \frac{556 \sqrt{861}}{2583} & \frac{80 \sqrt{21}}{63} \end{vmatrix} - 0 + 0. \]

So we only need to compute the $2 \times 2$ determinant:

\[ \begin{vmatrix} \frac{12 \sqrt{861}}{41} & 0 \\ \frac{556 \sqrt{861}}{2583} & \frac{80 \sqrt{21}}{63} \end{vmatrix}. \]

The determinant of this $2 \times 2$ matrix is

\[ \left(\frac{12 \sqrt{861}}{41}\right) \left(\frac{80 \sqrt{21}}{63}\right) - \left(0 \cdot \frac{556 \sqrt{861}}{2583}\right) = \frac{12 \sqrt{861}}{41} \cdot \frac{80 \sqrt{21}}{63}. \]

Now, simplify this expression:

\[ \frac{12 \sqrt{861}}{41} \cdot \frac{80 \sqrt{21}}{63} = \frac{12 \times 80 \times \sqrt{861} \times \sqrt{21}}{41 \times 63}. \]

Combine the constants and the square roots:

\[ \frac{960 \sqrt{861 \times 21}}{41 \times 63}. \]

Recall that $861 = 21 \times 41,$ so

\[ 861 \times 21 = (21 \times 41) \times 21 = 21^2 \times 41. \]

Thus 

\[ \sqrt{861 \times 21} = \sqrt{21^2 \times 41} = 21 \sqrt{41}. \]

Substitute this back into the expression:

\[ \frac{960 \times 21 \sqrt{41}}{41 \times 63}. \]

Now, simplify the fraction:

\[ \frac{960 \times 21 \sqrt{41}}{41 \times 63}. \]

Notice that $21$ in the numerator and $63$ in the denominator can be simplified since $63 = 3 \times 21$. Thus the fraction becomes

\[ \frac{960 \times 21 \sqrt{41}}{41 \times 63} = \frac{960 \times 21 \sqrt{41}}{41 \times 3 \times 21} = \frac{960 \sqrt{41}}{41 \times 3} = \frac{960 \sqrt{41}}{123}. \]

Simplifying $\frac{960}{123},$ we get

\[ \frac{960 \div 3}{123 \div 3} = \frac{320}{41}. \]

Thus the determinant is 

\[ \frac{320 \sqrt{41}}{41}. \]

Now, multiply this result by $\sqrt{41}$ from the expansion of the $3 \times 3$ determinant:

\[ \sqrt{41} \cdot \frac{320 \sqrt{41}}{41} = \frac{320 \times 41}{41} = 320. \]

Therefore, the volume $V$ is

\[ V = \frac{1}{6} \left| 320 \right| = \frac{320}{6} = \frac{160}{3}. \]

Now we have the volume $V = \frac{160}{3}$ and the total surface area $A_{\text{total}} = 24 \sqrt{21}$.

Using the formula for the inradius $r$:

\[ r = \frac{3V}{A_{\text{total}}} = \frac{3 \cdot \frac{160}{3}}{24 \sqrt{21}} = \frac{160}{24 \sqrt{21}} = \frac{20}{3 \sqrt{21}}. \]

Rationalize the denominator:

\[ r = \frac{20}{3 \sqrt{21}} \cdot \frac{\sqrt{21}}{\sqrt{21}} = \frac{20 \sqrt{21}}{3 \times 21} = \frac{20 \sqrt{21}}{63}. \]

Thus the inradius is $\frac{20 \sqrt{21}}{63}$. This is in the form $\frac{m \sqrt{n}}{p}$ where $m = 20$, $n = 21$, and $p = 63$. 

Therefore, $m + n + p = 20 + 21 + 63 = 104$.

Answer: 104



